Measurement of the total and leptonic decay widths of the $J/\psi$ resonance with an energy scan method at BESIII

Using $e^+e^-$ annihilation data sets collected with the BESIII detector, we measure the cross sections of the processes $e^+e^- \to e^+e^-$ and $e^+e^- \to \mu^+\mu^-$ at fifteen center-of-mass energy points in the vicinity of the $J/\psi$ resonance. By a simultaneous fit to the measured, center-of-mass energy dependent cross sections of the two processes, the combined quantities $\Gamma_{ee} \Gamma_{ee} / \Gamma_{\rm tot}$ and $\Gamma_{ee} \Gamma_{\mu\mu} / \Gamma_{\rm tot}$ are determined to be ($0.346 \pm 0.009$) and ($0.335 \pm 0.006$) keV, respectively, where $\Gamma_{ee}$, $\Gamma_{\mu\mu}$, and $\Gamma_{\rm tot}$ are the electronic, muonic, and total decay widths of the $J/\psi$ resonance, respectively. Using the resultant $\Gamma_{ee} \Gamma_{\mu\mu} / \Gamma_{\rm tot}$ and $\Gamma_{ee} \Gamma_{ee} / \Gamma_{\rm tot}$, the ratio $\Gamma_{ee} / \Gamma_{\mu\mu}$ is calculated to be $1.031 \pm 0.015$, which is consistent with the expectation of lepton universality within about two standard deviations. Assuming lepton universality and using the branching fraction of the $J/\psi$ leptonic decay measured by BESIII in 2013, $\Gamma_{\rm tot}$ and $\Gamma_{ll}$ are determined to be ($93.0 \pm 2.1$) and ($5.56 \pm 0.11$) keV, respectively, where $\Gamma_{ll}$ is the average leptonic decay width of the $J/\psi$ resonance.

==> AmsMathEnvForLineno.tex <==
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
  \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
  \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
  \renewenvironment{#1}%
     {\linenomath\csname old#1\endcsname}%
     {\csname oldend#1\endcsname\endlinenomath}}% 
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}


==> Event_Selection/exp_mc_cmpr_ee_and_mumu_nmnl_rslt_30969_pq_n.tex <==
\begin{figure}[!h]
\centering
\subfigure{\includegraphics[width=0.325\textwidth]{Event_Selection/eetoee/exp_mc_cmpr_ee_nmnl_rslt_30969_Pofchrgd_n.pdf}}
\subfigure{\includegraphics[width=0.325\textwidth]{Event_Selection/eetoee/exp_mc_cmpr_ee_nmnl_rslt_30969_Csthofchrgd_n.pdf}}
%\subfigure{\includegraphics[width=0.325\textwidth]{Event_Selection/eetoee/exp_mc_cmpr_ee_nmnl_rslt_30969_Eofchrgd_n.pdf}}
\subfigure{\includegraphics[width=0.325\textwidth]{Event_Selection/eetoee/exp_mc_cmpr_ee_nmnl_rslt_30969_EOPofchrgd_n.pdf}}
\subfigure{\includegraphics[width=0.325\textwidth]{Event_Selection/eetomumu/exp_mc_cmpr_mumu_nmnl_rslt_30969_Pofchrgd_n.pdf}}
\subfigure{\includegraphics[width=0.325\textwidth]{Event_Selection/eetomumu/exp_mc_cmpr_mumu_nmnl_rslt_30969_Csthofchrgd_n.pdf}}
%\subfigure{\includegraphics[width=0.325\textwidth]{Event_Selection/eetomumu/exp_mc_cmpr_mumu_nmnl_rslt_30969_Eofchrgd_n.pdf}}
\subfigure{\includegraphics[width=0.325\textwidth]{Event_Selection/eetomumu/exp_mc_cmpr_mumu_nmnl_rslt_30969_EOPofchrgd_n.pdf}}
\subfigure{\includegraphics[width=0.325\textwidth]{Event_Selection/eetomumu/exp_mc_cmpr_mumu_nmnl_rslt_30969_Deltatofofchrgds_n.pdf}}
\caption{\small Comparison between data and MC simulation of the distributions of the variables used in the selection criteria for the processes \eetoee and \eetomumu at $\sqrt{s}=3096.9$ MeV. For all the plots, dots with error bars show the background-subtracted data (the background level is evaluated with the MC simulation) and the histograms denote the signal MC. The small discrepancy in the last plot is due to the imperfection of the MC simulation, and it has a negligible effect on the cross section measurement of $e^+e^- \to \mu^+\mu^-$.}
\label{Figure: Comparisons between data and MC of the selection condition related distributions of signal candidates of eetoee and eetomumu at sqrts=3096.9 MeV after event selection.}
\end{figure}

